Can Self-Supervised Representation Learning Methods Withstand Distribution Shifts and Corruptions?

Self-supervised learning in computer vision aims to leverage the inherent structure and relationships within data to learn meaningful representations without explicit human annotation, enabling a holistic understanding of visual scenes. Robustness in vision machine learning ensures reliable and consistent performance, enhancing generalization, adaptability, and resistance to noise, variations, and adversarial attacks. Self-supervised paradigms, namely contrastive learning, knowledge distillation, mutual information maximization, and clustering, have been considered to have shown advances in invariant learning representations. This work investigates the robustness of learned representations of self-supervised learning approaches focusing on distribution shifts and image corruptions in computer vision. Detailed experiments have been conducted to study the robustness of self-supervised learning methods on distribution shifts and image corruptions. The empirical analysis demonstrates a clear relationship between the performance of learned representations within self-supervised paradigms and the severity of distribution shifts and corruptions. Notably, higher levels of shifts and corruptions are found to significantly diminish the robustness of the learned representations. These findings highlight the critical impact of distribution shifts and image corruptions on the performance and resilience of self-supervised learning methods, emphasizing the need for effective strategies to mitigate their adverse effects. The study strongly advocates for future research in the field of self-supervised representation learning to prioritize the key aspects of safety and robustness in order to ensure practical applicability. The source code and results are available on GitHub.

==> Qs.tex <==
\textbf{Q1: How do self-supervised learning (SSL) paradigms (contrastive learning, knowledge distillation, mutual information maximization, clustering) perform in terms of robustness when exposed to distribution shifts and image corruptions?}

The average error rates against all corruptions (per severity level) of all the SSL methods are depicted in Fig. \ref{fig:avg}. The general trend is that SimCLR and SimSam have higher error rates as compared to other methods. While Contrastive learning has reported good performance previously on ImageNet-C \cite{khosla2021supervised}, we noticed that SimCLR is not comparably robust against these corruptions, which should not discredit Contrastive methodologies. 

 \begin{figure}
     \centering
     \includegraphics[width=0.5\textwidth]{figs/Averages/average_all.png}
     \caption{Error rates vs. severity levels across ImageNet-C \cite{imagenetc} corruptions. 
 % need to elaborate much more
     }
     \label{fig:avg}
 \end{figure}

A pattern observed (Fig. \ref{fig:avg}) is that, in general, Knowledge distillation methods seem to outperform contrastive solutions, while information maximization is only on pare. The surprising success of clustering should indicate that a more extensive study is needed on the robustness of the various methods. From fig~\ref{fig:avg}, one important observation is that for corruptions with lower severity levels, six algorithms form three groups where SwaV and DINO perform best, followed by BYOL and Barlow twins; finally, SimCLR and SimSiam have relatively poorer performance. However, at the highest severity level, all the algorithms have similar error rates due to misclassification. This is likely because most images in this group are heavily distorted and challenging even for the human visual system to comprehend.
From Table~\ref{tab:overview}, we observe that SwaV outperforms all the competing methods in terms of corruption error and mean corruption error; however, DINO has a better clean error rate. 

\begin{table}[H]
% Transpose this
    \centering
    \caption{Results for each method calculated over the corruption metric \cite{imagenetc}. }
    \resizebox{0.45\textwidth}{!}{
    \begin{tabular}{l|rrrrrr}
        \hline
        {} &     Barlow Twin &       BYOL &     SimCLR &     SimSam &       SWaV &       DINO \\
        \hline
            Clean Error &   28.2 & 28.2 &   33.1 &   31.7 & 29.5 & \textbf{24.7} \\
            Average Error rate    &   73.8 & 73.8 &   75.99 &   75.8 & \textbf{70.5} & 71.5 \\
            Average Relative Error        &   74.7 & 74.6 &   76.0 &   76.0 & \textbf{70.7} & 72.9 \\ \hline

    \end{tabular}
    }    
    \label{tab:overview}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Q2: To what extent can self-supervised learning methods maintain their robustness in the presence of distribution shifts, and what are the factors that limit their ability to do so?}

Table~\ref{tab:overview_large} presents a detailed analysis using mean corruption error $mCE$ for each corruption. Here, we report the average $mCE$ for each corruption in the ImageNet-C dataset. For calculating the error rate, we have taken the average across each severity level $CE$ for a particular corruption type, as described in \eqref{eq:average_metric}. One of the findings is that glass blur significantly impacts the robustness of these models, specifically at higher severity levels. Most of these models have demonstrated good robustness to brightness-based corruptions. As corroborated by Fig.~\ref{fig:3-elst-sat-sno} for most corruptions, the model robustness suffers with the increase in severity levels.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/C_vs_Method/all_figs_1.png}
    \caption{Model performance against specific corruptions by severity. For corruptions, namely, snow, saturate, and elastic (last row), SSL models perform poorly at severity level 2 than at severity level 3.}
    \label{fig:3-elst-sat-sno}
\end{figure}

\begin{table}[h!]
    \centering
        \caption{$mCE$ for each corruption type against the baseline, as calculated in \eqref{eq:average_metric}. The error rates in each column of corruption types are average values of all severity levels.}
    \resizebox{1\textwidth}{!}{
   \begin{tabular}{lrrrrrrrrrrrrrrrrrrrr}
                                         & \multicolumn{1}{l}{}              & \multicolumn{4}{l}{\textbf{Weather}}                                        & \multicolumn{3}{l}{\textbf{Noise}}                             & \multicolumn{4}{l}{\textbf{Extra}}                                                             & \multicolumn{4}{l}{\textbf{Digital}}                                                          & \multicolumn{4}{l}{\textbf{Blur}}                                   \\ \hline
\multicolumn{1}{l|}{}                    & \multicolumn{1}{r|}{\textbf{mCE}} & \textbf{Snow} & \textbf{Frost} & \textbf{Fog} & \multicolumn{1}{r|}{\textbf{Bright}} & \textbf{Gauss.} & \textbf{Shot} & \multicolumn{1}{r|}{\textbf{Impulse}} & \textbf{Speckle} & \textbf{Gauss.} & \textbf{Spatter} & \multicolumn{1}{r|}{\textbf{Saturate}} & \textbf{Pixelate} & \textbf{Contrast} & \textbf{Elastic} & \multicolumn{1}{r|}{\textbf{JPEG}} & \textbf{Zoom} & \textbf{Defocus} & \textbf{Motion} & \textbf{Glass} \\ \hline
\multicolumn{1}{l|}{\textbf{barlow}}     & \multicolumn{1}{r|}{73.8}         & 84            & 78             & 87           & \multicolumn{1}{r|}{46}     & 73              & 75            & \multicolumn{1}{r|}{83}      & 70               & 73              & 69               & \multicolumn{1}{r|}{47}                & 66                & 85                & 72               & \multicolumn{1}{r|}{62}            & 86            & 79               & 80              & 88             \\
\multicolumn{1}{l|}{\textbf{byol}}       & \multicolumn{1}{r|}{73.8}         & 85            & 78             & 86           & \multicolumn{1}{r|}{46}     & 73              & 76            & \multicolumn{1}{r|}{81}      & 71               & 73              & 70               & \multicolumn{1}{r|}{48}                & 66                & 84                & 73               & \multicolumn{1}{r|}{63}            & 86            & 78               & 80              & 86             \\
\multicolumn{1}{l|}{\textbf{simclr}}     & \multicolumn{1}{r|}{76.0}         & 85            & 78             & 89           & \multicolumn{1}{r|}{48}     & 76              & 79            & \multicolumn{1}{r|}{85}      & 76               & 77              & 70               & \multicolumn{1}{r|}{50}                & 67                & 80                & 75               & \multicolumn{1}{r|}{68}            & 88            & 83               & 82              & 88             \\
\multicolumn{1}{l|}{\textbf{simsam}}     & \multicolumn{1}{r|}{75.8}         & 85            & 80             & 90           & \multicolumn{1}{r|}{50}     & 74              & 76            & \multicolumn{1}{r|}{81}      & 71               & 74              & 73               & \multicolumn{1}{r|}{50}                & 65                & 88                & 75               & \multicolumn{1}{r|}{63}            & 88            & 82               & 84              & 89             \\
\multicolumn{1}{l|}{\textbf{swav}}       & \multicolumn{1}{r|}{70.5}         & 80            & 73             & 79           & \multicolumn{1}{r|}{41}     & 71              & 73            & \multicolumn{1}{r|}{82}      & 68               & 70              & 65               & \multicolumn{1}{r|}{44}                & 67                & 73                & 71               & \multicolumn{1}{r|}{60}            & 83            & 77               & 77              & 85             \\
\multicolumn{1}{l|}{\textbf{dino}}       & \multicolumn{1}{r|}{72.9}         & 83            & 75             & 82           & \multicolumn{1}{r|}{41}     & 74              & 75            & \multicolumn{1}{r|}{84}      & 68               & 70              & 65               & \multicolumn{1}{r|}{44}                & 68                & 79                & 70               & \multicolumn{1}{r|}{60}            & 82            & 76               & 76              & 85             \\
\multicolumn{1}{l|}{\textbf{supervised}} & \multicolumn{1}{r|}{76.7}         & 78            & 75             & 66           & \multicolumn{1}{r|}{57}     & 80              & 82            & \multicolumn{1}{r|}{83}      & 76               & 74              & 76               & \multicolumn{1}{r|}{58}                & 77                & 71                & 85               & \multicolumn{1}{r|}{77}            & 80            & 75               & 78              & 89          \\ 
%\multicolumn{1}{l|}{\textbf{dino/vit-8s}} &\multicolumn{1}{r|}{57.3} & 59 & 56 & 70 & \multicolumn{1}{r|}{30} & 55 & 57 & \multicolumn{1}{r|}{61} &50 & 63 & 41 & \multicolumn{1}{r|}{32} & 54 & 75 & 51 & \multicolumn{1}{r|}{51} & 75 & 70 & 64 & 74 \\\hline
\end{tabular}
    }
    \label{tab:overview_large}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Q3: What is the relationship between the robustness performance of different SSL paradigms and common categories of corruptions? }
\textbf{TODO: calculate means for each group and add to the paper and discuss}














%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Q4: Do self-supervised learning methods deviate from the observed trend of error increase for certain corruptions, and what factors contribute to their robustness in the face of these corruptions?} 

From Fig.~\ref{fig:3-elst-sat-sno}, for three corruptions, namely, snow, saturate, and elastic transforms (last row), we find a deviation from the expected trend; the expected trend is that the error increases with an increase in severity level. However, SSL models are performing poorly at severity level 2 than at severity level 3. To investigate it further, we used the Structural Similarity Index measure (SSIM)~\cite{struct}, one of the metrics popularly used by image quality researchers for reference image-based quality assessment. 

%  \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figs/ssim_plot.png}
%     \caption{SSIM values over severity by corruption. Note that higher values indicate higher clarity in this context. As severity increases, the SSIM index should decrease. Snow and Elastic transform have shifts between severity levels 2 and 3, which could explain the result of the oddities viewed in Figure \ref{fig:3-elst-sat-sno}.}
%     \label{fig:ssim}
% \end{figure}

We computed the SSIM between the original image (from ImageNet) and the corresponding corrupted image (from ImageNet-C) for all test images and averaged at each severity level; this gives an estimate of the visual quality. The findings are given in Fig.\ref{fig:ssim}. 

%  \begin{table}[h]
% \centering
%     \caption{SSIM metric for snow, elastic and saturate-based corruptions.}
% \begin{tabular}{l|lll}
% \hline
% Severity & Snow            & Elastic    & Saturate            \\ \hline
% 1    & 0.218 & 0.276  & 0.288 \\
% 2    & 0.179  & 0.237 & 0.283  \\
% 3    & 0.194  & 0.315  & 0.273  \\
% 4    & 0.186  & 0.312  & 0.234  \\
% 5    & 0.189 & 0.305  & 0.210 \\ \hline
% \end{tabular}
%     \label{tab:ssim}
% \end{table}
Snow corruption occludes the object by adding whitish pixels as snowflakes with motion blur. It has more visually challenging images at severity level 2 than other levels; therefore, SSIM at level 2 is lower than the SSIM at other severity levels. 
Similarly, for elastic transform, the SSIM at level 2 is lower than the SSIM at other severity levels. At low severity (levels 1 and 2), the affine transform is more noticeable in some cases, causing artifacts, which can also be seen in figure \ref{fig:grad_rep_grid} on its elastic transform. 
The Saturation corruptions have no saturation at low severity levels, causing it to be a grayscale image. This might lead to some classes not being accurately predicted, where color information is crucial.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figs/ssim_plot.png}
    \caption{SSIM values over severity by corruption. Note that higher values indicate higher clarity in this context. As severity increases, the SSIM index should decrease. Snow and Elastic transform have shifts between severity levels 2 and 3, which could explain the result of the oddities viewed in Figure \ref{fig:3-elst-sat-sno}.}
    \label{fig:ssim}
    \includegraphics[width=0.8\textwidth]{figs/gradcams/dog_3.png}
    \caption{Glass blur on dogs; markers in the images show correct (green) and incorrect (red) classifications. In ImageNet with many dog breed classes, misclassification doesn't necessarily indicate a bad model if the representation is adequate. In the twin dog example, with low blur severity, both dogs have good activations for all models, suggesting good representations. However, at high blur severity, the model struggles to classify, resulting in distorted activations and difficulty in distinguishing between the dogs, leading to poor results.}
    \label{fig:grad_dog_grid}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Q5: To what extent does the presence of corruptions shift the focus of classifiers from overall representation to specific features?}

To gain more insight into how different self-supervised algorithms for classification pick a label, we have used gradcams~\cite{gradcam} to compare the different methods qualitatively. Gradcams are a widely used tool by computer vision researchers to explain the model's decision as they provide heatmaps on where in the image the model is focusing. 

In Fig~\ref{fig:grad_rep_grid}, we show the grad cams of an image for all SSL methods under different corruptions of varying severity levels. 
The difference among Gradcams gives an understanding of how the model behavior changes in the presence of a particular corruption. From Table~\ref{tab:overview_large}, we noticed that glass blur corruption had caused the highest misclassification for all competing SSL methods; to understand how different methods respond to different severity of glass blur, we provide the corresponding gradcams in Fig.~\ref{fig:grad_dog_grid}.
%Gradcam

\begin{figure}
        \centering
    \includegraphics[width=0.7\textwidth]{figs/gradcams/rep_2.png}
    \caption{Random Corruptions on a Cobra; the markers in the images show correct and incorrect classifications. Cobra, a reptile with multiple classes in ImageNet, may confuse classifiers. However, cobras are generally distinguishable from other reptiles due to their distinctive neckband. At severity level 2 of elastic transform, there are artifacts causing a distorted doublet, making it a challenging case. Overall, models perform well with good representation. The classifier in these examples shows a bias towards the neckband, while the original un-cropped image emphasizes the edges for classification by DINO and SwaV. However, due to corruptions, the focus shifts more towards the neckband.}
    \label{fig:grad_rep_grid}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Q6: Do different backbones, such as Convolutional Neural Networks (CNNs) and Transformers, influence the behavior and robustness?}


